Learning Multimodal Behaviors from Scratch with Diffusion Policy Gradient

Deep reinforcement learning (RL) algorithms typically parameterize the policy as a deep network that outputs either a deterministic action or a stochastic one modeled as a Gaussian distribution, hence restricting learning to a single behavioral mode. Meanwhile, diffusion models emerged as a powerful framework for multimodal learning. However, the use of diffusion policies in online RL is hindered by the intractability of policy likelihood approximation, as well as the greedy objective of RL methods that can easily skew the policy to a single mode. This paper presents Deep Diffusion Policy Gradient (DDiffPG), a novel actor-critic algorithm that learns from scratch multimodal policies parameterized as diffusion models while discovering and maintaining versatile behaviors. DDiffPG explores and discovers multiple modes through off-the-shelf unsupervised clustering combined with novelty-based intrinsic motivation. DDiffPG forms a multimodal training batch and utilizes mode-specific Q-learning to mitigate the inherent greediness of the RL objective, ensuring the improvement of the diffusion policy across all modes. Our approach further allows the policy to be conditioned on mode-specific embeddings to explicitly control the learned modes. Empirical studies validate DDiffPG's capability to master multimodal behaviors in complex, high-dimensional continuous control tasks with sparse rewards, also showcasing proof-of-concept dynamic online replanning when navigating mazes with unseen obstacles.

==> section/preliminary.tex <==


%\textbf{Policy Gradient Theorem}~~~The Policy Gradient Theorem (PGT) provides a foundation for continuous action reinforcement learning (RL) by optimizing the parameters $\theta$ of a policy $\pi_\theta(a|s)$ directly, by optimizing the expected return $J(\theta) = \mathop{\mathbb{E}}_{\pi_\theta}[R]$, where $R$ here denotes the cumulative reward. According to the \textit{Policy Gradient Theorem}~\citep{sutton1999policy}, the gradient of $J(\theta)$ w.r.t. the policy parameters $\theta$ is given by $
%\nabla_\theta J(\pi_\theta) = \mathop{\mathbb{E}}_{\pi_\theta}\left[\nabla_\theta \log \pi_\theta(a|s) \cdot Q^{\pi_\theta}(s, a)\right]
%$, i.e., we can adjust the policy parameters in the direction of the performance gradient $\nabla_\theta %J(\pi_\theta)$. This theorem forms the basis for many policy gradient methods~\citep{silver2014deterministic,wu2022understanding}. However, it suffers from the need to estimate reliably the action-value function $Q^{\pi_\theta}(s, a)$, with the simplest solution being the use of a sample return for estimating the $Q^\pi$, as in REINFORCE~\citep{williams1992simple}.

%\\
%\textbf{Actor-Critic Algorithms}~~~Actor-Critic algorithms represent a significant class of methods in RL, building upon the principles of PGT. These algorithms consist of two main components: the \textit{actor} and the \textit{critic}~\citep{schulman2015trust,mnih2016asynchronous,lillicrap2015continuous,haarnoja2018soft}. The actor is represented by a policy function $\pi_\theta(a|s)$, and the critic  evaluates the chosen actions using the action-value function $Q_\phi(s, a)$  parameterized by $\phi$. The critic serves as the approximation needed by PGT for guiding the updates of the actor. The learning process involves two simultaneous updates: one for the actor, using a policy gradient approach, and one for the critic, using temporal difference learning. By combining the exploratory policy updates of the actor with the value-based guidance of the critic, Actor-Critic algorithms aim to balance exploration and exploitation efficiently, enabling robust and effective policy learning in complex environments.

